The CHiME-7 DASR Challenge: Distant Meeting Transcription with Multiple Devices in Diverse Scenarios

The CHiME challenges have played a significant role in the development and evaluation of robust automatic speech recognition (ASR) systems. We introduce the CHiME-7 distant ASR (DASR) task, within the 7th CHiME challenge. This task comprises joint ASR and diarization in far-field settings with multiple, and possibly heterogeneous, recording devices. Different from previous challenges, we evaluate systems on 3 diverse scenarios: CHiME-6, DiPCo, and Mixer 6. The goal is for participants to devise a single system that can generalize across different array geometries and use cases with no a-priori information. Another departure from earlier CHiME iterations is that participants are allowed to use open-source pre-trained models and datasets. In this paper, we describe the challenge design, motivation, and fundamental research questions in detail. We also present the baseline system, which is fully array-topology agnostic and features multi-channel diarization, channel selection, guided source separation and a robust ASR model that leverages self-supervised speech representations (SSLR).

==> discarded.tex <==
\begin{table}[ht]
\centering
\footnotesize
\caption{Frame-level class frequency (\%), FA denotes segmentation obtained with forced alignment}\label{tab:class_stats}
\begin{tabular}{@{\extracolsep{0.5pt}}ccccccc}
\toprule   
 {Class frequency} & split  & 0-spk & 1-spk & 2-spk & 3-spk & 4-spk \\
\midrule
\multirow{3}{*}{CHi\-ME-6} & train & 22.59 & 53.48 & 18.43 & 4.28 & 1.20   \\
 & dev & 12.53  & 43.67  & 30.51  &  11.30   & 1.96 \\
& eval &  19.92  & 50.96  & 20.71  & 5.74  & 2.64  \\
\midrule
\multirow{3}{*}{CHi\-ME-6 FA} & train &  &  &  &  &    \\   
 & dev & 24.05  & 54.25  &  17.74  &  3.49   & 0.47  \\
& eval &     &   &   &   &   \\
\midrule
\multirow{2}{*}{DiPCo} & dev & 7.64 & 66.56 & 21.80 & 3.75 & 2.18  \\
& eval & 9.23 & 65.82 & 19.38 & 4.88 &  0.67 \\
\midrule
\multirow{2}{*}{Mixer 6} & dev & 3.05 & 76.18 & 20.75  &  -  &  - \\
& eval & 2.40  & 83.66 & 13.93 & - & - \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!htbp]
    \caption{CHiME-7 DASR results for each scenario: \ac{SA-WER} and \ac{GSS}+selection inference time versus EV top-k microphones used; (\%) of all available channels.}
    \label{tab:detailed_ev}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{2.5pt}
    \begin{tabular}{clcccc}
    
    \hline
         \textbf{Top-k (\%)} & \textbf{Scenario} & \multicolumn{2}{c}{{ \textbf{Dev}}} &  \multicolumn{2}{c}{ \textbf{Eval}}\\
         & & SA-WER  & Time   & SA-WER  & Time  \\
           & & (\%)  & (h:mm)  &   (\%) & (h:mm) \\
         \hline
            \multirow{3}{*}{100} & CH\-iME-6 &  36.1   & 1:53  &  38.9   & 3:30  \\
                                &  DiPCo &    40.0    & 1:10  &  41.5     &  1:10 \\
                                & Mixer 6 & 22.3     & 1:48  &  27.0   & 0:52 \\ 
        \hline
            \multirow{3}{*}{80} & CH\-iME-6 &  35.3  & 1:25  & 38.4  &  2:58 \\
                                &  DiPCo &  37.0  &  0:53  & 40.3   & 0:46 \\
                                & Mixer 6 &  23.1  & 1:32  & 29.5  & 0:31 \\ 
        \hline
            \multirow{3}{*}{60} & CH\-iME-6 &  36.2  & 1:12 &    38.6   & 2:12 \\
                                &  DiPCo &   36.7  & 0:38 & 40.3    & 0:29  \\
                                & Mixer 6 &  23.8  & 1:16 &  33.8   & 0:19  \\ 

        \hline
            \multirow{3}{*}{40} & CH\-iME-6 &  39.8  &  0:49 &   40.2   & 1:30 \\
                                &  DiPCo &   37.7  & 0:21 &    42.0    &   0:19 \\
                                & Mixer 6 &  25.5    & 0:59 &   36.0     & 0:18  \\ 
        \hline
            \multirow{3}{*}{20} & CH\-iME-6 & 49.9  & 0:36 &  48.7    &  1:05 \\
                                &  DiPCo &  41.6  & 0:16 &   47.1  & 0:15 \\
                                & Mixer 6 & 27.6  & 0:46 &  37.4   & 0:14 \\ 
        \hline
    \end{tabular}
  
\end{table} 







\begin{table}[t]
    \caption{CHiME-7 DASR optional sub-track results obtained using the best configuration from development set (80\% channels GSS). Results are in terms of \% WER.}
    \label{tab:final_results}
    \centering
    \begin{tabular}{@{}llcc@{}}
    \toprule
         \textbf{ASR} & \textbf{Scenario} & \textbf{Dev} &   \textbf{Eval} \\ 
    \midrule
    \multirow{4}{*}{Whisper} & CH\-iME-6 &    35.7  &  40.7 \\
                                &  DiPCo & 37.8  &   39.7    \\
                                & Mixer 6 &  22.9   &    25.2   \\ 
                                 \cmidrule{2-4}
                                & \textbf{Macro} &   32.1    & 35.2  \\
    \midrule
    \multirow{4}{*}{\textbf{Ours}} & CH\-iME-6 &  32.2  &    \\
                                &  DiPCo &    &       \\
                                & Mixer 6 &    &    \\ 
                                 \cmidrule{2-4}
                                & \textbf{Macro} &    &   \\ 
    \bottomrule
    \end{tabular}
\end{table}

